Accelerated Inference in Markov Random Fields via Smooth Riemannian Optimization

Markov Random Fields (MRFs) are a popular model for several pattern recognition and reconstruction problems in robotics and computer vision. Inference in MRFs is intractable in general and related work resorts to approximation algorithms. Among those techniques, semidefinite programming (SDP) relaxations have been shown to provide accurate estimates while scaling poorly with the problem size and being typically slow for practical applications. Our first contribution is to design a dual ascent method to solve standard SDP relaxations that takes advantage of the geometric structure of the problem to speed up computation. This technique, named Dual Ascent Riemannian Staircase (DARS), is able to solve large problem instances in seconds. Our second contribution is to develop a second and faster approach. The backbone of this second approach is a novel SDP relaxation combined with a fast and scalable solver based on smooth Riemannian optimization. We show that this approach, named Fast Unconstrained SEmidefinite Solver (FUSES), can solve large problems in milliseconds. Contrarily to local MRF solvers, e.g., loopy belief propagation, our approaches do not require an initial guess. Moreover, we leverage recent results from optimization theory to provide per-instance sub-optimality guarantees. We demonstrate the proposed approaches in multi-class image segmentation problems. Extensive experimental evidence shows that (i) FUSES and DARS produce near-optimal solutions, attaining an objective within 0.1% of the optimum, (ii) FUSES and DARS are remarkably faster than general-purpose SDP solvers, and FUSES is more than two orders of magnitude faster than DARS while attaining similar solution quality, (iii) FUSES is faster than local search methods while being a global solver.

==> app-params.tex <==
%!TEX root = main.tex
\section*{Appendix E: \fuses and \dars parameters}
\label{sec:results:params}
The parameters for \fuses and \dars are listed below.
\input{table-parameters}

==> app-proof-SDP2.tex <==
%!TEX root = main.tex

\section*{Appendix C: Proof of~\prettyref{prop:newSDP2}}
\label{sec:proof:prop:newSDP2}

The proof that $\fsdpopt \leq \fsdpoptTwo$ follows from the fact that the two problems have the same objective 
and the feasible set of~\eqref{eq:newSDP2} is a subset of the feasible set~\eqref{eq:newSDP} (the former includes two extra constraints, 
$\MZ \geq 0$ and $[\MZ]_{tr} \ones_{\nrClasses}=\ones_{\nrNodes}$). 
Next we prove that the SDP~\eqref{eq:newSDP2} is also a convex relaxation of~\eqref{eq:homBinaryMat}
and $\fsdpoptTwo \leq \fopt$. Towards this goal we note that~\eqref{eq:homBinaryMat} can be rewritten as:
%
\beq
\begin{array}{rcl}
\fopt = & \min_{\MV} & \trace{\MV\tran \MQ \MV}  \\
&\subject   & \diag{[\MV \MV\tran]_{tl}} = \ones_{\nrNodes}  \\
&	       & [\MV \MV\tran]_{br} = \eye_{\nrClasses}  \\
&           & \MV\in\{0,1\}^{(\nrNodes+\nrClasses)\times(\nrClasses)}\\
&          & [\MV \MV\tran]_{tr} \ones_{\nrClasses}=\ones_{\nrNodes} \\
&          & \MV \MV\tran \geq 0
\end{array}
\eeq
%
where we added two redundant constraints ($\MV \MV\tran \geq 0$ and $[\MV \MV\tran]_{tr} \ones_{\nrClasses}=\ones_{\nrNodes}$) to~\eqref{eq:homBinaryMat}. These two constraints are always satisfied in~\eqref{eq:homBinaryMat} 
since $\MV \MV\tran$ is always a nonnegative matrix ($\MV \MV\tran \geq 0$) when $\MV$ is a binary matrix, 
and since $[\MV \MV\tran]_{tr} \ones_{\nrClasses}=\ones_{\nrNodes} \overset{{\tiny\text{using~\eqref{eq:homogenization2}}}}{=} \MX \ones_{\nrClasses}=\ones_{\nrNodes}$ 
(this is a redundant constraint imposing one label per node). 
At this point, it is straightforward to repeat the same derivation we used to get~\eqref{eq:newSDP} (i.e., substitute $\MZ = \MV \MV\tran$ and drop the rank-$\nrClasses$ constraint on $\MZ$) 
and get the relaxation~\eqref{eq:newSDP2}. This proves that~\eqref{eq:newSDP2} is a convex relaxation of~\eqref{eq:homBinaryMat}
and $\fsdpoptTwo \leq \fopt$, concluding the proof.
% We first prove that $$
%  Intuitively, we added extra constraints to~\eqref{eq:newSDP} (which makes $\fsdpopt \leq \fsdpoptTwo$), 
%  and those constraints are always satisfied by~\eqref{eq:homBinaryMat} (making~\eqref{eq:newSDP2} a convex relaxation of the MAP estimator). 

% In~\eqref{eq:newSDP2} we notice that the entries of $\MZ$ must be non-negative. 
% Therefore, we restricted the optimization to \emph{doubly nonnegative matrices} $\MZ$.\footnote{A doubly nonnegative matrix is 
% a symmetric matrix with non-negative entries.} Moreover, we noticed that each row in the top-right block of $\MZ$, \cf with eq.~\eqref{eq:homogenization2},
% should sum up to 1.

==> app-results-randomInitialization.tex <==
%!TEX root = main.tex

\section*{Appendix D: Additional results}
\label{sec:results:additionalResults}

In this section, we provide the complete statistics of the experiments reported in table \ref{table-statistics-lindau-1000} and \ref{table-statistics-lindau-2000}. 

The results are generated using default initialization schemes for each approach. To further demonstrate the advantage of using our global solvers, we perform another experiment by using the same random initialization for all techniques and keeping all other setting the same. 


==> experimentsEmpty.tex <==
%!TEX root = main.tex

\section{Experiments}
\label{sec:experiments}

\mbox{}
\newpage

\mbox{}
\newpage

\mbox{}
\vspace{15cm}


==> fig-segmentation-snapshots.tex <==
%!TEX root = main.tex

\newcommand{\myhspace}{\hspace{0mm}}

\newcommand{\mpw}{4cm}
\begin{figure}[t]
\vspace{-5mm}
	\begin{center}
	\hspace{-0.4cm}
		\begin{minipage}{\textwidth}
			\begin{tabular}{ccccc}%
			\myhspace
				\begin{minipage}{\mpw}%
				\centering
				\includegraphics[width=1.05\columnwidth]{gray} \\
				(a) Bonnet \fuses 
				\end{minipage}
			& \myhspace
				\begin{minipage}{\mpw}%
				\centering%
				\includegraphics[width=1.05\columnwidth]{gray} \\
				(b) \fuses  
				\end{minipage}
			& \myhspace
				\begin{minipage}{\mpw}%
				\centering%
				\includegraphics[width=1.05\columnwidth]{gray} \\
				(c)  \dars  
				\end{minipage}
			\end{tabular}
		\end{minipage}%
		\vspace{-2mm}
		\caption{Snapshots of the semantic segmentation produced by 
		(a) Bonnet, (b) \fuses, and (c) \dars, on the Cityscapes dataset.\label{fig-segmentation-snapshots}}
		\vspace{-10mm} 
	\end{center}
\end{figure}

